AI-SAM: Automatic and Interactive Segment Anything Model

Semantic segmentation is a core task in computer vision. Existing methods are generally divided into two categories: automatic and interactive. Interactive approaches, exemplified by the Segment Anything Model (SAM), have shown promise as pre-trained models. However, current adaptation strategies for these models tend to lean towards either automatic or interactive approaches. Interactive methods depend on prompts user input to operate, while automatic ones bypass the interactive promptability entirely. Addressing these limitations, we introduce a novel paradigm and its first model: the Automatic and Interactive Segment Anything Model (AI-SAM). In this paradigm, we conduct a comprehensive analysis of prompt quality and introduce the pioneering Automatic and Interactive Prompter (AI-Prompter) that automatically generates initial point prompts while accepting additional user inputs. Our experimental results demonstrate AI-SAM's effectiveness in the automatic setting, achieving state-of-the-art performance. Significantly, it offers the flexibility to incorporate additional user prompts, thereby further enhancing its performance. The project page is available at https://github.com/ymp5078/AI-SAM.

==> latex_figs/ablation_heatmaps.tex <==
\begin{figure}[ht!]
\centering % Centers the entire figure

\begin{tikzpicture}[scale=0.8]
% First heatmap
\begin{axis}[
    width=0.65\linewidth,
    height=0.65\linewidth,
    view={0}{90},
    xlabel=Random 4 Point,
    ylabel=Prompt Feature,
    % title=Confusion Matrix Heatmap,
    colormap={bluewhite}{color=(white) rgb255=(90,96,191)}, % Use the 'Blues' colormap
    xtick={0,...,3},
    ytick={0,...,3},
    xticklabels={None, RV, Myo, LV},
    yticklabels={None, RV, Myo, LV},
    enlargelimits=false,
    axis on top,
    xticklabel style={anchor=north, rotate=0},
    yticklabel style={anchor=south, rotate=90},
    axis line style={draw=none},tick style={draw=none}, % Remove the tick marks but keep the tick labels
    mesh/cols=4, % Number of columns in the data matrix
    mesh/rows=4, % Number of rows in the data matrix
    point meta min=0, % Minimum value for color data
    point meta max=1, % Maximum value for color data
    nodes near coords align={anchor=center},
    nodes near coords={\pgfmathprintnumber[/pgf/number format/fixed]\pgfplotspointmeta},
]

% Matrix plot with numbers on top
\addplot[matrix plot*, point meta=explicit] table [meta=C] {
    x y C
    0 0 0.5831
    1 0 0.4607
    2 0 0.5398
    3 0 0.5277
    0 1 0.5293
    1 1 0.772
    2 1 0.6498
    3 1 0.6388
    0 2 0.539
    1 2 0.6374
    2 2 0.8586
    3 2 0.8362
    0 3 0.5258
    1 3 0.5902
    2 3 0.8384
    3 3 0.9051
};
\end{axis}

% Second heatmap (copy of the first one)
\begin{axis}[
    at={(0.5\linewidth,0)}, % This shifts the second plot to the right of the first one
    width=0.65\linewidth,
    height=0.65\linewidth,
    view={0}{90},
    xlabel=AI-Prompter 4 Points,
    % ylabel=True class,
    % title=Confusion Matrix Heatmap,
    colormap={bluewhite}{color=(white) rgb255=(90,96,191)}, % Use the 'Blues' colormap
    xtick={0,...,3},
    xtick={0,...,3},
    ytick={0,...,3},
    xticklabels={None, RV, Myo, LV},
    yticklabels={},
    enlargelimits=false,
    axis on top,
    tick label style={font=\small},
    xticklabel style={anchor=north, rotate=0},
    yticklabel style={anchor=south, rotate=90},
    axis line style={draw=none},tick style={draw=none}, % Remove the tick marks but keep the tick labels
    mesh/cols=4, % Number of columns in the data matrix
    mesh/rows=4, % Number of rows in the data matrix
    point meta min=0, % Minimum value for color data
    point meta max=1, % Maximum value for color data
    nodes near coords align={anchor=center},
    nodes near coords={\pgfmathprintnumber[/pgf/number format/fixed]\pgfplotspointmeta},
]

% Matrix plot with numbers on top (second copy)
\addplot[matrix plot*, point meta=explicit] table [meta=C] {
    x y C
    0 0 0.5636
    1 0 0.4372
    2 0 0.5122
    3 0 0.5123
    0 1 0.5304
    1 1 0.7783
    2 1 0.6477
    3 1 0.6274
    0 2 0.54
    1 2 0.5511
    2 2 0.8527
    3 2 0.835
    0 3 0.5261
    1 3 0.6088
    2 3 0.836
    3 3 0.8865
};

\end{axis}
\begin{axis}[
    at={(0,0.5\linewidth)}, % This shifts the second plot to the right of the first one
    width=0.65\linewidth,
    height=0.65\linewidth,
    view={0}{90},
    % xlabel=Class Feature,
    ylabel=Output Feature,
    % title=Confusion Matrix Heatmap,
    colormap={bluewhite}{color=(white) rgb255=(90,96,191)}, % Use the 'Blues' colormap
    xtick={0,...,3},
    ytick={0,...,3},
    xticklabels={},
    yticklabels={None, RV, Myo, LV},
    enlargelimits=false,
    axis on top,
    xticklabel style={anchor=north, rotate=0},
    yticklabel style={anchor=south, rotate=90},
    axis line style={draw=none},tick style={draw=none}, % Remove the tick marks but keep the tick labels
    mesh/cols=4, % Number of columns in the data matrix
    mesh/rows=4, % Number of rows in the data matrix
    point meta min=0, % Minimum value for color data
    point meta max=1, % Maximum value for color data
    nodes near coords align={anchor=center},
    nodes near coords={\pgfmathprintnumber[/pgf/number format/fixed]\pgfplotspointmeta},
]

% Matrix plot with numbers on top
\addplot[matrix plot*, point meta=explicit] table [meta=C] {
    x y C
    0 0 0.9993
    1 0 0.0003
    2 0 0.0004
    3 0 0.0
    0 1 0.3119
    1 1 0.6581
    2 1 0.0214
    3 1 0.0086
    0 2 0.2539
    1 2 0.0164
    2 2 0.6914
    3 2 0.0383
    0 3 0.1648
    1 3 0.0015
    2 3 0.0314
    3 3 0.8023
};
\end{axis}

% Second heatmap (copy of the first one)
\begin{axis}[
    at={(0.5\linewidth,0.5\linewidth)}, % This shifts the second plot to the right of the first one
    width=0.65\linewidth,
    height=0.65\linewidth,
    view={0}{90},
    % xlabel=Class Feature,
    % ylabel=True class,
    % title=Confusion Matrix Heatmap,
    colormap={bluewhite}{color=(white) rgb255=(90,96,191)}, % Use the 'Blues' colormap
    xtick={0,...,3},
    ytick={0,...,3},
    xticklabels={},
    yticklabels={},
    enlargelimits=false,
    axis on top,
    tick label style={font=\small},
    xticklabel style={anchor=north, rotate=0},
    yticklabel style={anchor=south, rotate=90},
    axis line style={draw=none},tick style={draw=none}, % Remove the tick marks but keep the tick labels
    mesh/cols=4, % Number of columns in the data matrix
    mesh/rows=4, % Number of rows in the data matrix
    point meta min=0, % Minimum value for color data
    point meta max=1, % Maximum value for color data
    nodes near coords align={anchor=center},
    nodes near coords={\pgfmathprintnumber[/pgf/number format/fixed]\pgfplotspointmeta},
]

% Matrix plot with numbers on top (second copy)
\addplot[matrix plot*, point meta=explicit] table [meta=C] {
    x y C
    0 0 0.9992
    1 0 0.0004
    2 0 0.0004
    3 0 0.0
    0 1 0.1944
    1 1 0.7274
    2 1 0.0582
    3 1 0.0201
    0 2 0.1001
    1 2 0.0186
    2 2 0.8313
    3 2 0.05
    0 3 0.0312
    1 3 0.0021
    2 3 0.0442
    3 3 0.9225
};

\end{axis}

\end{tikzpicture}

\caption{The Output Confusion Metric (Top Row) and the Prompt Confusion Metric (Bottom Row) using AI-SAM feature on ACDC dataset.}
\label{fig:abl_conf_mat}
\end{figure}

==> latex_figs/ablation_n_points.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    % title={Line Plot Example},
    xlabel={Points / Class},
    ylabel={DICE\%},
    xmin=0, xmax=17,
    ymin=91.5, ymax=92.4,
    xtick={1,2,4,8,16},
    ytick={91.5, 91.7, 91.9, 92.1, 92.3},
    ylabel style={
        rotate=0,
        yshift=-3pt, % Adjust this value to move the ylabel closer or further
        font=\small
    },
    xlabel style={
        rotate=0,
        yshift=3pt, % Adjust this value to move the xlabel closer or further
        font=\small
    },
    yticklabel style={
        rotate=45,% Rotate the y-axis tick labels
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd,
        % xshift=1pt,
        font=\small
    },
    ticklabel style={font=\small, inner sep=2pt}, % Reduce space by setting inner sep
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
    width=\linewidth,  % Set the width of the plot
    height=0.5\linewidth, % Set the height of the plot
    axis lines=left,
]

\addplot[
    color=blue,
    mark=*,
    ]
    coordinates {
    (1,92.17)(2,92.25)(4,92.06)(8,92.05)(16,91.77)
    };
    % \legend{Data Series}

% Add a vertical line at x=4
\draw [red, thick, dashed] (axis cs:4,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs:4,\pgfkeysvalueof{/pgfplots/ymax});
% Add the text "SAM #Points" at (4,92.2)
\node [above] at (axis cs:6.5,91.7) {SAM \#Points};

\end{axis}
\end{tikzpicture}
\caption{The ablation study on the number of prompt points. The red dashed line denote the maximum number of point SAM is trained on.}
\label{fig:num_points}
\end{figure}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
